QRES: Quantitative Reasoning on Encrypted Security SLAs

While regulators advocate for higher cloud transparency, many Cloud Service Providers (CSPs) often do not provide detailed information regarding their security implementations in their Service Level Agreements (SLAs). In practice, CSPs are hesitant to release detailed information regarding their security posture for security and proprietary reasons. This lack of transparency hinders the adoption of cloud computing by enterprises and individuals. Unless CSPs share information regarding the technical details of their security proceedings and standards, customers cannot verify which cloud provider matched their needs in terms of security and privacy guarantees. To address this problem, we propose QRES, the first system that enables (a) CSPs to disclose detailed information about their offered security services in an encrypted form to ensure data confidentiality, and (b) customers to assess the CSPs' offered security services and find those satisfying their security requirements. Our system preserves each party's privacy by leveraging a novel evaluation method based on Secure Two Party Computation (2PC) and Searchable Encryption techniques. We implement QRES and highlight its usefulness by applying it to existing standardized SLAs. The real world tests illustrate that the system runs in acceptable time for practical application even when used with a multitude of CSPs. We formally prove the security requirements of the proposed system against a strong realistic adversarial model, using an automated cryptographic protocol verifier.

==> src/1-authors.tex <==
\author[1]{Alice Smith}
\author[2]{Bob Jones}
\affil[1]{Department of Mathematics, University X}
\affil[2]{Department of Biology, University Y}

\maketitle

==> src/1-qese-protocol.tex <==
\begin{figure*}
\begin{center}
\fbox{
\pseudocode{
\textbf{Provider} (\p) \< \< \textbf{Broker} (\broker)  \\[0.1\baselineskip]
 {knowledge: } \<\<{knowledge: }\\
\sk_{\p},\pk_{\p},\pk_{\broker}, \key, \kpvauth,\sigma_{\p}^{auth},c^{t^1}_{\p},\ldots, c^{t^n}_{\p} \< \<\sk_{\broker},\pk_{\broker}, \kpvauth,\sigma_{\p}^{auth}, {w^{1}_{\cust}},\ldots, {w^{n}_{\cust}}, c^{t^1}_{\p},\ldots, c^{t^n}_{\p} \\[0.1\baselineskip][\hline]
 \<\< \\[-0.5\baselineskip]
   \textbf{[7]} \hspace{0.1cm} \gar_\key\leftarrow \enc(\key,x) \<\sendmessageright*[2cm]{\gar_\key} \< \textbf{[8]} \hspace{0.1cm} \text{Using \textit{OT:} } \\
\< \<  G^{w^{1}_{{\cust}}} \leftarrow w^{1}_{{\cust}}  \\
 \< \< \sig(\sk_{\cust},G^{w^{1}_{{\cust}}}) \leftarrow \sig(\sk_{\cust},{w^{1}_{{\cust}}})\\
\< \< \textbf{[9]} \hspace{0.1cm} \vrfy(\pk_{\cust},\sig(\sk_{\cust},G^{w^{1}_{{\cust}}}) \text{ valid?}\\
 \< \< \textbf{[10]} \hspace{0.1cm} c^{G^{w^{1}_{\cust}}}\sample \gar_\key(G^{w^{1}_{{\cust}}})\\  
  \< \< \hspace{0.1cm} c^{G^{w^{1}_{\cust}}} \coloneqq \enc(\key, w^{1}_{{\cust}}) \\
\< \< \textbf{[11]} \hspace{0.1cm} d \sample \search(c^{w^1_{\cust}},c^{t^1}_{{\p}},\ldots, c^{t^n}_{{\p}})\\
}
}
\end{center}
\caption{Secure computation protocol}
  \label{fig:full}
\end{figure*}



==> src/2-abstract1-N.tex <==
%!TEX root = ../template.tex

\begin{abstract}{
Although the  European Commission  has put forth regulations for higher cloud transparency,   many Cloud Service Providers (CSPs) do not provide detailed information regarding their  security implementations  in their  Service Level Agreements (SLAs). 
In practice,CSPs are hesitant to release detailed information regarding their security posture for security and proprietary reasons.
Since the SLA works as an agreement between the customer and the CSP, customers cannot get security guarantees regarding the offered services.
This lack of transparency  hinders the adoption of cloud computing by enterprises and individuals. 
To address this problem, we propose QRES, the first system that enables (a) CSPs to publicly disclose their encrypted security SLAs (secSLAs) and (b)  customers to \textit{privately assess} the CSPs' offered security services and find those satisfying their security requirements. 
Our system preserves each party's privacy by leveraging  technologies  such as Secure Two Party Computation (2PC) and Searchable Encryption.
We implement  QRES and  highlight its usefulness by applying it to existing standardized SLAs. 
The real world tests illustrate that the system runs in acceptable time for practical application even when used with a multitude of CSPs.
We formally prove the  security requirements of the proposed system against a strong realistic adversarial model, using an automated cryptographic protocol verifier.
}
\end{abstract}


\journalname{Proceedings on Privacy Enhancing Technologies}
\DOI{Editor to enter DOI}
\startpage{1}
\received{..}
\revised{..}
\accepted{..}

\journalyear{..}
\journalvolume{..}
\journalissue{..}


\keywords{Cloud Security, Privacy Preserving Systems, Security Service Level Agreements}{}

\maketitle

==> src/3-Intro-revised-N.tex <==
\section{Introduction}

Cloud computing enables customers to develop, manage, and access a spectrum of Cloud resources (computing, storage, applications, etc.) which are typically offered as-a-service in a remotely accessible manner. Albeit the numerous claimed benefits of the Cloud to ensure confidentiality, integrity, and availability of the stored data, the number of security breaches is still on the rise \cite{popa2011enabling, secBr}. The absence of security claims verification has constrained the customers from confiding in the CPSs, hence limiting the full potential use of their services. Unless CSPs disclose detailed security-related information about their security offers, the customers cannot verify that their security requirements will be met.

Security-related information can be interpreted as any information that can assist the CSPs to identify, assess, monitor, and respond to security threats \cite{NISTIS}.  For example: (a) security alerts and procedures for vulnerability discovering, reporting and remediation, (b) security controls and configuration elements, and (c) information on software updates and patches to be applied \cite{ENISA, NISTIS}. Using this information, customers can evaluate CSPs offered security services and compare different service offerings provided by numerous CSPs in order to find the best CSP satisfying their requirements; characteristically, security services are defined as the CSP's level of security based on the implemented security controls. %to assess the CPSs security level, customers can evaluate CSPs offered security posture\footnote{Security posture is defined as the CSP's level of security based on the implemented security controls.} and also compare different service offerings provided by varied CSPs in order to find the best CSP satisfying their security requirements. 
%Using this information, customers can assess CSPs offered security posture and compare different service offerings provided by various CSPs in order to find the best CSP satisfying their requirements

In this context, a number of Cloud stakeholders\footnote{For example, the European Network and Information Security Agency (ENISA) \cite{enisa11}, Cloud Security Alliance (CSA) \cite{csa11}, and, ISO/IEC \cite{ISO}} have advocated that defining the security services in security Service Level Agreements (named security SLA or simply secSLA \cite{jesus2015}) can help establish common semantics to provide and manage security assurance. Consequently, secSLAs can be a beneficial mean not only to share information about each CSP offered security services, but also to define the services' key measurable parameters (e.g., how a CSP recovers from incidents is typically defined in terms of the incident severity and the time to recovery \cite{ENISA}). Customers can employ these measurable parameters to continuously evaluate and monitor (even with a realistic level of automation) the CSP's implementation of the acquired service level.

Meanwhile, the European Commission has put forth regulations mandating higher Cloud transparency (e.g., the European Union's Cyber Security Framework \cite{cybersec}). The incentives of sharing information on a CSP's security services across the customers and also other CSPs transpire as:
\begin{enumerate}[-]
\item Customers can use this information to assess the CSPs to be able to ascertain the level of security service they purchase.
\item Economic incentives stemming from the reputation benefits of CSPs sharing their offered security services.
\end{enumerate}

Notwithstanding the benefits of disclosing information on their security services, the CSPs still do not wish to publicly share highly sensitive information\footnote{For example, detailed information about the key measurable parameters of the offered services, vulnerability management/assessment procedures, and commercial offers} for security and/or commercial apprehensions such as:

\begin{enumerate}[-]
 \item Publicly detailing commercial sensitive information (i.e., financial terms, service levels, cost information, vulnerability descriptions which may include proprietary information, etc.) can be used by other competitors to their advantage.
% 
 \item Publicly sharing the sensitive information about the CSPs vulnerabilities and/or security parameters may increase the rate of malicious security breaches which leads to a significant reputation and financial loss.
%\item Competitors can exploit such highly sensitive information (i.e., financial terms, service levels, cost information, vulnerability descriptions which may include proprietary information, etc.).
%\item Loss of reputation on sharing the CSP's vulnerabilities and/or security parameters, which could potentially lead to further security breaches.
\end{enumerate}

In this paper, we propose QRES (Quantitative  Reasoning on Encrypted  SLAs), as a formally verified approach, that solves the CSPs and customers seemingly conflicting needs with respect to sharing the CSP's security services. We attain the aforementioned by allowing (a) CSPs to disclose detailed information of the security services offered in their secSLAs and then encrypt the secSLAs to ensure confidentiality, and (b) customers to explore their security requirements over the CSP's encrypted secSLAs and determine the best CSP matching their requirements.

\subsection{Challenges and contributions}

Building such a system is challenging as:

\textbf{P1:} The Customers' cannot search through the encrypted secSLAs, unless their requirements are also encrypted with the same secret key used by each CSP to encrypt its secSLA. Consequently, the system should uphold the desired secSLA's confidentiality requirements through allowing the customers to search their requirements blindly without neither the CSPs learning them, nor the customers obtaining the CPS's secret key.

\textbf{P2:} The system should prevent malicious CSPs from deliberately providing false information to match the customer requirements. 

\textbf{P3:}  The system should forbid malicious customers to verify information about each CSP offered services (i.e., by performing various searching iterations, each iteration with different requirements).

To address these problems, \textit{QRES} allows customers (or a broker on behalf of the customers) to search over CSPs encrypted secSLAs (as depicted in Figure \ref{fig:RA}) utilizing a novel security enhanced two-party privacy preserving query over an encrypted data scheme (named \textit{QeSe}) such that:  
\begin{enumerate}[I)]
	\item \textit{QeSe} uses a searchable encryption scheme along with a novel evaluation method. The evaluation method utilizes the exact-matching privacy model which finds and evaluates the services exactly matching the customer requirements (tackling P1).
	\item \textit{QeSe} supports a new security property by enhancing the security setting of the traditional two-party privacy preserving computation (Yao garbled circuit evaluation \cite{yao1986generate,lindell2009proof}\footnote{Yao garbled circuit is explained in Section \ref{sec:SC}} is the one used in this paper). This is achieved by validating the participants' inputs (i.e., CSP's secSLA and customer requirements) before computation (tackling P2 \& P3).	 
\end{enumerate} 

%\begin{enumerate}[I)]
%	\item \textit{QeSe} uses a searchable encryption scheme along with an exact matching privacy model and a proposed evaluation method which finds and evaluates the services exactly matching the customer requirements (tackling P1)	
%	\item \textit{QeSe} enhances the security setting of the traditional two-party privacy preserving computation by validating the participants' inputs (i.e., CSP's secSLA and customer requirements) before computation (tackling P2 \& P3)	
%\end{enumerate} 


To verify the \textit{QRES} system correctness\footnote{\textit{QRES} must ensure that the entities should learn nothing except their output and each entity should receive its correct output.}, we start by formally defining the required security properties (cf., Section \ref{sec:Req}). Further, we conduct a formal security analysis of \textit{QRES} using ProVerif~\cite{blanchet2001efficient}, an automated cryptographic protocol verifier, establishing the defined properties against a strong adversarial model (i.e., Dolev-Yao adversary model \cite{dolev1983security}).


To validate our system model, we implement \textit{QRES} using Amazon AWS DynamoDB \cite{ddb} and also based on actual CSP security related information found on the publically available STAR (Security, Trust and Assurance Registry) \cite{csa_star} repository, which are compliant with the ISO/IEC 19086 standard \cite{iso19086}. Our rationale behind using STAR repository is that (i) to the best of our knowledge, no other Cloud secSLA repositories are publicly available and (ii) major CSPs are still in the process of restructuring their secSLAs by leveraging the recently published ISO/IEC 19086.

\begin{figure}[h]
\centering 
%\includegraphics[width=11cm,height=6.5cm]{./img/System.pdf} 
\scalebox{0.28}{\includegraphics{./img/System-new1.pdf}}
\squeezeup
%\squeezeup
\caption{\textit{QRES} System Model}
  \label{fig:RA}
\end{figure}

\subsubsection*{{\textbf{Contributions. }}}
Summarizing our contributions:
\begin{enumerate}
\item We propose the first formally established complete system (\textit{QRES}) which achieves both the customer and CSP requirements regarding sharing the CSPs security services, while addressing the outlined problems P1, P2 \&P3.
\item We use ProVerif to formally prove the correctness of \textit{QRES} by defining the needed security properties and establishing that the system holds these properties against a strong adversarial model. 
\item We implement \textit{QRES} and evaluate the system using real-world CSP secSLAs. We demonstrate that \textit{QRES} performance is appropriate for the presented use case. 
\end{enumerate}

The ProVerif scripts and proofs used in this paper as well as the system implementation are publicly available at \cite{qres}. 


\subsection{{Outline}}
The rest of the paper is organized as follows: Section \ref{sec:RA} defines the system and threat models, as well as the system objectives and requirements. The basic concepts of the cryptographic tools, notations, and security definitions used are developed in Section \ref{sec:notation}. Section \ref{sec:SA} elaborates the architecture of the proposed system. %The proposed ranking scheme is presented in Section \ref{sec:rank}. 
The implementation of the presented system is detailed in Section \ref{sec:imp}. A security analysis of the \textit{QRES} system is presented in Section \ref{sec:SC}. Finally, we present our conclusions in Section \ref{sec:conc}.



==> src/3-Intro.tex <==
\section{Introduction}

Cloud computing allows customers to develop, manage, and access a spectrum of Cloud resources (storage, software, applications, etc.) which are offered as-a-service in a remotely accessible fashion. In such a service-based environment, the Cloud provisioning relies on stipulated Service Level Agreement (SLA). These SLAs specify the Cloud service levels requested by the customers, and required to be achieved by the Cloud Service Providers (CSPs). %Furthermore, CSPs have the opportunity to offer the same services at different service and financial levels according to the set of customers (i.e., corporate, individual customer, etc.), in the same SLA. 
%
Despite the various benefits of the Cloud, the number of data breaches are increasing every year. The lack of security assurance and transparency has prevented customers and enterprises from trusting the CSPs, and hence not using their services. Unless the customers security requirements are identified, documented, and communicated by the CSPs, customers can not be assured that the CSPs will satisfy their requirements.

In this context, a number of Cloud community stakeholders (e.g., ISO 27002 \cite{ISO}, the European Network and Information Security Agency (ENISA) \cite{enisa11}, and Cloud Security Alliance (CSA) ~\cite{csa11}) have advocated that defining the security parameters in SLAs can establish common semantics to provide and manage security assurance. Consequently, SLA can be a useful mean not only to disclose information about each CSP offered services, but also to define the services' key measurable parameters\footnote{For example, how a CSP recovers from incidents is typically defined in terms of: the incident severity and the time to recovery~\cite{ENISA}}.

The customers can use the key measurable parameters to assess and monitor the CSP's implementation of %security measures of 
the acquired service level. Using these assessments customers have better information to compare different service offerings provided by various CSPs and then select the best CSP that satisfies their requirements. Examples of security related information that can be included in SLAs are (a) security controls and configuration elements (e.g., metrics for measuring cybersecurity performance), (b) information on software updates and patches to be applied, and (c) procedures for vulnerability discovering, reporting and remediation \cite{ENISA}. 

Despite the benefits of these kind of information, still CSPs do not disclose detailed information about (a) the key measurable parameters of the offered services, and (b) vulnerability management/assessment procedures, in their public SLAs for security and/or commercial reasons \cite{ENISA} such as:
\begin{enumerate}[-]
 \item Publicly detailing commercial sensitive information (i.e., financial terms, service levels, cost information, vulnerability descriptions which may include proprietary information, etc.) can be used by other competitors to improve their services.
 \item Publicly disclosing security parameters may assist attackers to penetrate the system using a hole in the publicized data. Accordingly, the rate of malicious security breaches increases, which can be much harder to detect. This can also lead to a significant financial loss as a result of the customers compensation. 
\end{enumerate}
%

Therefore, a system that simultaneously allows:
\begin{enumerate}[(R1)] 
\item CSPs to specify their services along with the key measurable parameters in their SLAs, without revealing information about the offered security parameters and commercial sensitive information.
\item Customers to assess the CSP's offered services and choose the best CSP which satisfy their requirements, is needed. 
%
\end{enumerate}
In this paper, we propose \textit{QRES} (Quantitative Reasoning on Encrypted SLAs), the first formally proved complete system that solves the aforementioned challenges and achieves both of the seemingly conflicting properties (R1\&R2). This is achieved by allowing (a) CSPs to disclose their service controls in the SLAs and then encrypt their SLAs to ensure data confidentiality, and (b) customers to search for their requirements over the CSPs encrypted SLAs and find the best CSP matching their requirements. 

However, building such a system is challenging as:

\textbf{(P1)} The system should maintain the desired SLA privacy requirements by allowing the customers to obtain the encrypted search queries (specifying their requirements) without allowing, neither the CSPs to learn these queries nor the customers to know the CSP's secret key\footnote{Note that, the customers can only search over the encrypted SLAs, if their search queries are encrypted with the same secret key used by each CSP to encrypt its SLA.}. 

\textbf{(P2)} The system should prevent malicious customers to ascertain information about each CSP offered services (i.e., by performing several searching iterations, each iteration with different requirements or by performing frequency analysis). Furthermore, prevent malicious CSPs from deliberately providing false information to match the customer requirements. 

%\item Finally, how to ensure the privacy and correctness\footnote{The privacy requirement states that entities should learn nothing except their output. The correctness requirement states that each entity should receive its correct output.} of such a system?   

To tackle these problems, 
\textit{QRES} allows the customers (or a broker on behalf of the customers\footnote{In this paper, we assume the case of a novice or basic customer who can not search for her/his over encrypted data.}) to search over ``anonymous'' CSPs encrypted SLAs according to their requirements (as depicted in Figure \ref{fig:RA} and explained in Section \ref{sec:RA}). The searching scheme uses a proposed query searching scheme (named \textit{QeSe}) such that:  

\begin{enumerate}[-]
	\item \textit{QeSe} uses a searchable encryption scheme along with an exact matching privacy model and a proposed evaluation method which finds and evaluates the services exactly matching the customer requirements and nothing else.	
	\item \textit{QeSe} utilizes Yao garbled circuit \cite{yao1986generate,lindell2009proof} and oblivious transfer \cite{naor1999oblivious,asharov2013more} (cf., Section \ref{sec:SC}) to allow customers to find the best matching CSP's SLA without knowing the CSP's encryption key. At the same time, allowing CSPs to encrypt the customer search queries without learning these queries (tackling P1). 
	
	\item To prevent malicious customers from learning information about CSPs' SLAs, \textit{QeSe} allows the customers to lookup their requirements over ``anonymous'' CSPs encrypted SLAs.  The CSPs anonymity mitigates the malicious customers attacks as customers learn the result of the searching queries and nothing else. This means that the customer learns only the matching CSPs without knowing to which CSP each encrypted SLA belongs (tackling P2). \textit{QeSe} runs over an onion routing \cite{reed1998anonymous} anonymity network to ensure anonymity of CSPs.
\end{enumerate} 	

To verify the \textit{QRES} system correctness\footnote{\textit{QRES} must ensure that the entities should learn nothing except their output and each entity should receive its correct output.}, we start by formally defining the required security properties; the presented system must ensure the following privacy requirements: data confidentiality, data integrity, and CSP's anonymity (cf., Section \ref{sec:Req}). Further, we conduct a formal security analysis of \textit{QRES} using ProVerif~\cite{blanchet2001efficient}, an automated cryptographic protocol verifier, establishing the defined properties against a strong adversarial model.
 
%	check the existence of inconsistent requirements and/or preferences (tackling (P4), cf., Section ??), and (ii) rank the CSPs according to their requirements and priorities (tackling (P5), cf., Section \ref{sec:rank}).
%
%To tackle (P1), we utilize Yao garbled circuit \cite{yao1986generate,lindell2009proof} and oblivious transfer \cite{naor1999oblivious,asharov2013more} in the proposed system. 

%security and privacy properties of \textit{QRES}.  

To validate our system model we implement \textit{QRES} based on a real-world CSPs' SLAs found on the public STAR (Security, Trust and Assurance Registry) \cite{csa_star} repository, which are complaint with the relevant ISO/IEC 19086 standard \cite{iso19086}. 
We implement our system using Amazon AWS DynamoDB \cite{ddb} and Tor \cite{torpro}. The rationale for using STAR repository is that (i) to the best of our knowledge no other Cloud SLA repositories are publicly available and (ii) major CSPs are still in the process of restructuring their SLAs by leveraging the recently published ISO/IEC 19086\footnote{The ISO/IEC 19086 standard has been published Q3/2016, and it is expected to be adopted by major CSPs (and probably certifiable) by Q2/2018}.  

The ProVerif scripts and proofs used in this paper as well as the system implementation are publicly available at \cite{qres}. We show that \textit{QRES} performance is practical for the presented use case. 
\begin{figure}[h]
\centering 
%\includegraphics[width=11cm,height=6.5cm]{./img/System.pdf} 
\scalebox{0.28}{\includegraphics{./img/System-new1.pdf}}
%\squeezeup
%\squeezeup
\caption{\textit{QRES} System Model}
  \label{fig:RA}
\end{figure}

\subsection{{Contributions}}
Summarizing, our contributions are as follows.
\begin{enumerate}
\item We propose the first formally proved complete system (\textit{QRES}) which achieves both the R1\&R2 requirements while tackling the outlined problems (P1\&P2).
\item We formally prove the \textit{QRES} system correctness by defining the needed security properties and proving that the system holds these properties against a strong adversarial model using ProVerif.
\item We implement \textit{QRES} and evaluate the system using real-world CSPs' SLAs. We show that \textit{QRES}'s performance is practical for the presented use case.
\end{enumerate}

\subsection{{Outline}}
The rest of the paper is organized as follows: Section \ref{sec:RA} defines the system and threat models, as well as the system objectives and requirements. The basic concepts of the cryptographic tools, notations, and security definitions used are developed in Section \ref{sec:notation}. Section \ref{sec:SA} elaborates the architecture of the proposed system. The proposed ranking scheme is presented in Section \ref{sec:rank}. The implementation and the security analysis of the presented system is detailed in Section \ref{sec:impval}. A formal analysis of the \textit{QRES} system is presented in Section \ref{sec:FA}, and contrast our approach to related work in Section \ref{sec:sota}. Finally, we present our conclusions in Section \ref{sec:conc}.




==> src/9-ranking2.tex <==
\subsection*{Stage 7: CSPs Ranking.} 

Finally, the $\p$s are evaluated and ranked according to the number of tokens matching the customer requirements as described in the next section.
%
%However, this ranking scheme only checks which $\p$ can best satisfy the customer requirements without taking the customer priorities into consideration. To compare two or more $\p$s, customers should specify their priorities of each security service along with their requirements. In this paper, we propose an evaluation and ranking scheme named Prioritized keyword search schemes, as described in the next section.
\section{Evaluation and Ranking Schemes}
\label{sec:rank}
In this paper we consider two different evaluation schemes.
\subsection{Boolean Keyword Searching Scheme} The $\p$ with maximum number of encrypted tokens matching the customer keywords is given the highest score and selected as the best matching provider. However, this ranking scheme only checks which $\p$ can best satisfy the customer required values without taking the customer service preferences into consideration. To compare two or more $\p$s, the relative importance levels of the customer requirements for each service should be considered. 

\subsection{Prioritized Keyword Searching Scheme}
In this scheme, we allow the customers to assign the levels of importance (i.e., priorities) of each service along with her/his requirements. Hence, each customer sends her/his assigned priorities (named as priority list $weight_{w_{\cust}}$) along with her/his requirements during the keywords transfer (Stage 5). 
The $\p$s ranking is performed in the following progressive steps:

\subsubsection{Step A. Weights Assignment}
In order to rank different $\p$s, the importance levels of the customer requirements for each service are assigned as weights. We utilize qualitative terms to specify the importance of each service, where customers can assign qualitative terms to each service to indicate their priorities (\textit{Highly-Important(HI)}, \textit{Low-Important(LI)}, and \textit{Not-Required(NR)}). These qualitative terms are further transformed to a quantitative values. %($2,1,0$ respectively). 

%\begin{flalign*}
%    weight_{w_{\cust}}= 
%  \begin{bmatrix}
%weight_{w_{\cust}^1}, \ldots, weight_{w_{\cust}^n}
%  \end{bmatrix}
%\end{flalign*}
\subsubsection{Step B. Services Quantification}
In order to assess the $\p$s ($\p_i$) according to the customer requirements, a measurement model that considers each $\p$s' tokens which match the customer requirements using a pairwise relation is defined. 

For $m$ CSPs ($\p_i$), each $\p$ generates $n$ tokens $t_{\p}^n$. Further, a customer who generates $n$ keyword $w_{\cust}^n$ representing her/his requirements along with her/his priority list $weight_{w_{\cust}}$. A boolean value $V^{w_{\cust}}_{\p_i}$ is defined using pairwise relation of each customer encrypted keyword and $m$ $\p$s' encrypted tokens. $V^{w_{\cust}}_{\p_i}$ is true (equals to 1) if for each keyword, the exact match model returns a matching token so that:

\begin{flalign} 
\label{tfneq}
V^{w_{\cust}}_{t_{\p_i}^n}= \enc(\key_i, w_{\cust})/ \enc(\key_i, t_{\p_i}^n)
\end{flalign}
Thus,
\begin{flalign*} 
V^{w_{\cust}}_{t_{\p_i}^n}=
\begin{cases}
    1,& \text{if } \enc(\key_i, w_{\cust}) = \enc(\key_i, t_{\p_i}^n) \\
    0,& \text{if } \enc(\key_i, w_{\cust}) \neq \enc(\key_i, t_{\p_i}^n)  
   \end{cases}
\end{flalign*}

Thus, for each customer keyword (e.g., $w_{\cust}^1$) an evaluation matrix $(EM)$ is generated with size $m \times n$, if there is a total of $m$ CSPs each with $n$ tokens:

\begin{flalign}
EM_{w_{\cust}^1}= \bbordermatrix{&t^1&t^2&\ldots &t^n\cr
               \p_{1}& V^{w_{\cust}^1}_{t_{\p_1}^1} &V^{w_{\cust}^1}_{t_{\p_1}^2} & \ldots &V^{w_{\cust}^1}_{t_{\p_1}^n}\cr            
                     \vdots & \vdots & \vdots & \ddots& \vdots\cr       
                    \p_{m}&V^{w_{\cust}^1}_{t_{\p_m}^1}&V^{w_{\cust}^1}_{t_{\p_m}^2}& \ldots &V^{w_{\cust}^1}_{t_{\p_m}^n}}             
\end{flalign}

Similarly, we calculate $EM$ for each keyword of $n$ keywords ($EM_{w_{\cust}^1}, \ldots, EM_{w_{\cust}^n}$). Then, the relative ranking of all the $\p$s tokens for each keyword is calculated as a normalized vector of the $EM$ (named evaluation vector $EV$):



$EV_{w_{\cust}^1}=$
\small
\begin{flalign*}
\bbordermatrix{
  & \dfrac{V^{w_{\cust}^1}_{t_{\p_1}^1}}{( V^{w_{\cust}^1}_{t_{\p_1}^1}+\ldots +V^{w_{\cust}^1}_{t_{\p_m}^1})} &+\ldots &\dfrac{V^{w_{\cust}^1}_{t_{\p_1}^n}}{( V^{w_{\cust}^1}_{t_{\p_1}^n} +\ldots +V^{w_{\cust}^1}_{t_{\p_m}^n})}\cr
     &\vdots & \ddots& \vdots\cr
       &\dfrac{V^{w_{\cust}^1}_{t_{\p_m}^1}}{( V^{w_{\cust}^1}_{t_{\p_1}^1}+\ldots +V^{w_{\cust}^1}_{t_{\p_m}^1})} &+\ldots &\dfrac{V^{w_{\cust}^1}_{t_{\p_m}^n}}{( V^{w_{\cust}^1}_{t_{\p_1}^n} +\ldots V^{w_{\cust}^1}_{t_{\p_m}^n})}}
        \end{flalign*}
\normalsize

%
%%

As a result, 
\begin{flalign}
\label{eq:ev}
EV_{w_{\cust}^1}=\bbordermatrix{&\p_1&\p_2&\ldots &\p_m \cr
&N^{{w_{\cust}^1}}_{\p_1} & N^{{w_{\cust}^1}}_{\p_2} & \ldots & N^{{w_{\cust}^1}}_{\p_m}}
\end{flalign}
%%


%\begin{flalign*}
%EM= \bbordermatrix{&w_{\cust}^1&w_{\cust}^2&\ldots &w_{\cust}^n\cr
%               \p_{1}& V^{w_{\cust}^1}_{\p_1} &V^{w_{\cust}^2}_{\p_1} & \ldots &V^{w_{\cust}^n}_{\p_1}\cr            
%                     \vdots & \vdots & \vdots & \ddots& \vdots\cr       
%                    \p_{m}&V^{w_{\cust}^1}_{\p_m}&V^{w_{\cust}^2}_{\p_m}& \ldots &V^{w_{\cust}^n}_{\p_m}}             
%\end{flalign*}
%%%
%%
%%\begin{flalign*}
%%EV_{c^o_{\cust}}=\bbordermatrix{
%%  \p_{1}& \dfrac{V^{w_{\cust}^1}_{\p_1}}{( V^{w_{\cust}^1}_{\p_1}+\ldots +V^{w_{\cust}^1}_{\p_m})} &+\ldots +&\dfrac{V^{w_{\cust}^n}_{\p_1}}{( V^{w_{\cust}^n}_{\p_1} +\ldots +V^{w_{\cust}^n}_{\p_m})}\cr
%%     \vdots&\vdots & \ddots& \vdots\cr
%%   \p_{m}&\dfrac{V^{w_{\cust}^1}_{\p_m}}{( V^{w_{\cust}^1}_{\p_1}+\ldots +V^{w_{\cust}^1}_{\p_m})} &+\ldots +&\dfrac{V^{w_{\cust}^n}_{\p_m}}{( V^{w_{\cust}^n}_{\p_1} +\ldots +V^{w_{\cust}^n}_{\p_m})}}
%%\end{flalign*}
%%%%%

where $N^{{w_{\cust}^1}}_{\p_1}$ is a numerical value representing the relative rank of $\p_1$ to other CSPs regarding ${w_{\cust}^1}$.
%
\subsubsection{Step C. Services Aggregation}
The $EV$ is aggregated with the customer defined weights (assigned at Step A) to get the final ranking of the $\p$s as indicated by the ratios of numerical values.
\begin{flalign*}
EV_{w_{\cust}^1}^{agg}=
  EV_{w_{\cust}^1}. \begin{bmatrix}
weight_{w_{\cust}} 
  \end{bmatrix}^{T}  
\end{flalign*}
%
where $EV_{w_{\cust}^1}^{agg}$ is the aggregated vector which shows the final ranking of all the $\p$s based on the customer-defined requirements and weights. 

After finding the best matching $\p$, the selected $\p$'s authentication secret ($\kpvauth$) is sent to the auditor in order to identify the $\p$ identity. Next, the auditor sends the selected $\p$'s identity to $\broker$ which manages the agreement between both the $\p$ and $\cust$. 




